Data Assimilation with Machine Learning Surrogate Models: A Case Study with FourCastNet

Modern data-driven surrogate models for weather forecasting provide accurate short-term predictions but inaccurate and nonphysical long-term forecasts. This paper investigates online weather prediction using machine learning surrogates supplemented with partial and noisy observations. We empirically demonstrate and theoretically justify that, despite the long-time instability of the surrogates and the sparsity of the observations, filtering estimates can remain accurate in the long-time horizon. As a case study, we integrate FourCastNet, a weather surrogate model, within a variational data assimilation framework using partial, noisy ERA5 data. Our results show that filtering estimates remain accurate over a year-long assimilation window and provide effective initial conditions for forecasting tasks, including extreme event prediction.

==> plots.tex <==

\begin{figure*}
  \centering
  \includegraphics[width=13.5cm]{visualize_filtering_factor18_all_features_part1.png}
  \caption{Visualization of the ground truth ERA5 data, interpolated $4.5^\circ$ ERA5 observations with standardized $N(0,0.0001 I_{d_y})$ distributed additive errors, and our 3DVar analysis using this observational data and FourCastNet for 10 different atmospheric features at the end of our assimilation horizon, December 31, 2023 at 18:00 UTC.} \label{fig:assim_all_features_part1}
\end{figure*}

\begin{figure*}
  \centering
  \includegraphics[width=13.5cm]{visualize_filtering_factor18_all_features_part2.png}
  \caption{Visualization of the ground truth ERA5 data, interpolated $4.5^\circ$ ERA5 observations with standardized $N(0,0.0001 I_{d_y})$ distributed additive errors, and our 3DVar analysis using this observational data and FourCastNet for 10 different atmospheric features at the end of our assimilation horizon, December 31, 2023 at 18:00 UTC.} \label{fig:assim_all_features_part2}
\end{figure*}


\begin{figure*}
  \centering
  \includegraphics[width=15cm]{mawar_ws_ens_forecast_obs4.5.png}
  \caption{Visualization of three ensemble members' 48 hour forecasts of 10m wind speed for May 25, 2023 using three different initializations: noisy ground truth ERA5 data, noisy interpolated $4.5^\circ$ observations, and a 3DVar analysis ($4.5^\circ$ observations). For visual reference, we include ground truth ERA5 10m wind speed on May 25, 2023.} \label{fig:mawar_ws_ens}
\end{figure*}

\begin{figure*}
  \centering
  \includegraphics[width=15cm]{mawar_pressure_ens_forecast_obs4.5.png}
  \caption{Visualization of three ensemble members' 48 hour forecasts of mean sea level pressure for May 25, 2023 using three different initializations: noisy ground truth ERA5 data, noisy interpolated $4.5^\circ$ observations, and a 3DVar analysis ($4.5^\circ$ observations). For visual reference, we include ground truth ERA5 10m wind speed on May 25, 2023.} \label{fig:mawar_pressure_ens}
\end{figure*}


